Learning Shape Templates with Structured Implicit Functions

Template 3D shapes are useful for many tasks in graphics and vision, including fitting observation data, analyzing shape collections, and transferring shape attributes. Because of the variety of geometry and topology of real-world shapes, previous methods generally use a library of hand-made templates. In this paper, we investigate learning a general shape template from data. To allow for widely varying geometry and topology, we choose an implicit surface representation based on composition of local shape elements. While long known to computer graphics, this representation has not yet been explored in the context of machine learning for vision. We show that structured implicit functions are suitable for learning and allow a network to smoothly and simultaneously fit multiple classes of shapes. The learned shape template supports applications such as shape exploration, correspondence, abstraction, interpolation, and semantic segmentation from an RGB image.

==> fig/fig_3d_tsne.tex <==
\begin{figure*}[h!]
    \includegraphics[width=0.4\textwidth]{image/tsne/wide_dense/teaser1.png}
    \caption{A range of shapes from the ShapeNet~\cite{chang2015shapenet} database, fit to a structured implicit template, and arranged by template parameters using t-SNE~\cite{vanDerMaaten2008tsne}. Similar shape classes, such as airplanes, cars, and chairs, naturally cluster according to template parameters.}
    \label{fig:3d_tsne}
\end{figure*}

==> fig/fig_intraclass_mds.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{image/intraclass_mds/airplane_isosurface_quadrics.png}%
    \caption{Template consistency with a class. A sampling of templates fit to }
    \label{fig:multiclass_examples}
\end{figure}

==> fig/fig_real_images.tex <==
\begin{figure}[t]
    \centering
    \begin{tabular}{ccc}
    \includegraphics[width=0.9in, align=c]{image/real_images/71d0zTLR-NL.png} &
    \includegraphics[width=0.9in, align=c]{image/real_images/121474158955_1.JPG} &
    \includegraphics[width=0.9in, align=c]{image/real_images/141031368524_0.JPG}\\
    
    \includegraphics[width=0.9in, align=c]{image/real_images/71d0zTLR-NL_render.png} &
    \includegraphics[width=0.9in, align=c]{image/real_images/121474158955_1_render.png} &
    \includegraphics[width=0.9in, align=c]{image/real_images/141031368524_0_render.png} \\
    \includegraphics[width=0.9in, align=c]{image/real_images/141491110640_1.JPG} &
    \includegraphics[width=0.9in, align=c]{image/real_images/141493284932_0.JPG} &
    \includegraphics[width=0.9in, align=c]{image/real_images/181809603924_1.JPG}\\

    \includegraphics[width=0.9in, align=c]{image/real_images/141491110640_1_render.png} &
    \includegraphics[width=0.9in, align=c]{image/real_images/141493284932_0_render.png} &
    \includegraphics[width=0.9in, align=c]{image/real_images/181809603924_1_render.png}\\
    \end{tabular}
    \caption{Predictions from real images. \TODO{Make better renders, possibly by manually aligning the cameras. If we can add segmentations, that might be even better.} }
    \label{fig:real_images}
\end{figure}

==> sections/1_intro.tex <==
\section{Introduction}

\input{fig/fig_teaser.tex}

As multimedia databases based on 
3D shape collections become larger and more diverse, 
there is a growing need for automatically learned shape 
abstractions that can be used 
for analysis \cite{li2017grass}, exploration \cite{laga2017modeling},
correspondence \cite{XXX}, retrieval \cite{theologou2017part},
decomposition \cite{araslanov2016efficient}, 
decimation \cite{salinas2015structure}, and manipulation \cite{yumer2014co}.  For example, 
shape abstractions could be used for XXX and XXX
(Figure \ref{fig:teaser}).

For these applications, 
the goal of abstraction is to decompose 3D shapes
into human interpretable geometric elements and to establish 
relationships between the elements automatically.  For
example, when given a XXX and XXX as input, an abstraction
with consistently labeled shape elements could be used to \
XXX (Figure \ref{fig:teaser}).

Generating abstractions automatically for arbitrary shapes 
is a difficult task.  Traditional approaches have 
fit templates \cite{ganapathi2018parsing}, 
extracted geometric primitives \cite{tulsiani2017learning}, 
and/or segmented semantic parts \cite{yi2017learning}.
These methods have generally been able to produce only
small sets of shape elements (e.g., 3-6 boxes in \cite{tulsiani2017learning}), with limited
shape variation (e.g., 21 templates in \cite{ganapathi2018parsing}), 
for models trained separately on different object classes.
The goal of our work is to learn an unsupervised model that generates
detailed, consistent shape abstractions for all members of a diverse collection.  
Doing so requires an abstraction that can seamlessly blend between
shapes of different topology, part structure, and geometric complexity.

In this paper, we investigate using ``structured implicits'' as a 
learned shape representation for abstraction.  Structured implicits 
describe an 3D function as a composition of 
locally-supported 3D functions (shape elements), and an isolevel 
of the composition defines the inside/outside and surface of a shape.  
In our formulation, local shape elements are Gaussian functions
centered at arbitrary 3D positions and 
scaled anisotropically; however,
other functions could work as well (e.g., polynomials).  The main advantage
of this representation is that it supports continuous blends between
disparate shape structures and topologies, and thus is amenable to
learning with deep networks.

Our model for generating structured implicits is  
based on an encoder-decoder architecture (Figure \ref{fig:architecture}), 
where an encoder converts an observation 
(e.g., RGB image(s), RGBD image(s), 3D point cloud, 3D voxels, etc.) 
to a latent vector in a shape space,
and our decoder generates a structured implicit with a fixed
number of elements ($K=100$) from the latent vector.  The decoder
generates a set of Gaussian shape elements, whose sum produces
an implicit function that directly provides a classifier for
inside/outside.  The network is trained with a differentiable 
loss that penalizes misclassification of point samples as 
inside/outside, which can be backpropagated through the parameters
of the implicits and the weights in the network.

\TODO{Summary of results and applications}

Contributions



==> sections/3_learning_structured_implicits.tex <==
\section{Learning Structured Implicits}
\input{tab/table_representation_properties.tex}


We want to represent 3D shape in a way that is fundamentally compatible with both shape abstraction and learning. This is motivated by a natural synergy between abstraction and shape generating networks, which find continuous relationships between shapes by default.  So if we can find a suitable explicit representation and learn it, variation in the explicit representation will be similarly smooth and consistent.  In the results section, we also show that it is abstract in a semantically meaningful way.

More concretely, we want to learn a representation that has the right set of properties to support abstraction. In Table~\ref{tab:representation_properties}, frequently learned representations are shown in columns. Their properties as it relates to learning are shown in rows.

Abstract: decomposes a shape into conceptual elements.
Interpret: human interpretable.
Compact: data prop to surface complexity
Surface: loss based on surface reconstruction
Volume: loss based on inside/outside.
Topology: Continuity of topology changes
Articul: Continuity of surface motion?
Detail: Detail you can get from current methods


1. Describe what structured implicits are (come up with some general technical formulation). Describe them as a composition of implicit functions. 
\subsection{Representation Details}
We now seek to implement a basic form of structured implicits that still supports abstraction. The generality of the structured implicit formulation means that there are a variety of options. One popular and simple option, often referred to as ``Metaballs'' in the graphics literature, uses independent gaussian functions for the local functions and summation for the composition operator. Convolution surfaces~\cite{bloomenthal1991convolution} are another option, although in this representation the local functions are tied into skeletons via splines or polygons. This link could make the learning process more complex. The partition-of-unity implicits representation~\cite{ohtake2003multi} is also an option-- here the primitives are quadric surfaces and the composition operation is a gaussian-weighted partition-of-unity. We experimented with this representation but found the normalization in the composition operator to make learning less stable. The potentially more sophisticated interactions between quadric surfaces were also difficult to take advantage of in practice.

Therefore we opt for a variation of Metaballs. We include a generalization by making the radius anisotropic, which we found to help in accurately fitting thin structures. An even more general representation that includes arbitrary multivariate gaussian covariance matrices might do better with off-axis straight lines, although we do not experiment with this here.  

Formally, our representation is composed of local shape labeled $i\in [N]$, where $N$ is the number of implicits. Each local implicit $i$ has a center $p_i \in \mathcal{R}^3$, a radius $r_i \in \mathcal{R}^3$, and an always-negative constant $c_i \in \mathcal{R}^-$. Each local implicit defines an exponentially decaying function over all of space:
\begin{equation}
    f_i(x) = c_i \exp\left({\sum_{d \in \{x,y,z\}} \dfrac{(p_{i,d} - x_d)^2}{-2r_{i,d}^2} }\right)
\end{equation}.

The composition function for the local implicits is a sum. Therefore, the global function $F(x)$ representing the shape is
\begin{equation}
    F(x) = \sum_{i \in [N]} f_i(x)
\end{equation}
Because all constants $c_i$ are negative, we have that $\forall x \in \mathcal{R}^3 f_i(x) < 0$, and similarly $\forall x \in \mathcal{R^3} \sum_i f_i < 0$. Therefore we pick a negative isolevel $\ell$ and define the surface $S$ to be its crossing:
\begin{equation}
    S = \left\{ x  \in \mathcal{R}^3 : F(x)  = \ell\right\}
\end{equation}

We set $\ell := -0.07$, which was chosen by grid search. The reason that the constants are negative rather than positive is to maintain the convention that function values inside the surface should be less than $\ell$, while values outside the surface should be greater than $\ell$. This leads to a convenient 0/1 inside/outside test for points $x$:

\begin{equation}
    \sum_{i \in [N]} f_i(x) > \ell
\end{equation}

During training, a smoothed out inside/outside function is helpful for backpropogation:

\begin{equation}
    \mathrm{Sigmoid}\left(\alpha \sum_{i \in [N]}f_i(x)\right)
    \label{eq:soft_classification}
\end{equation}

Above, $\alpha$ defines the degree of smoothing out to be applied to the inside/outside query. 

One final note is that for most experiments presented here, we use $N = 100$. Because each implicit requires 7 constants, the total dimensionality of our representation is a fixed $7N = 700$ floating point values. This fixed dimensionality is helpful both for efficiently training networks and for maintaing smooth correspondence between abstract shape elements. \TODO{Maybe this last part goes in the previous subsection.}

==> sections/3_shape_representation.tex <==
\section{Structured Implicit Shape Representation}

We assume each input shape can be modeled as a watertight surface bounding an interior volume (real-world meshes usually must be processed to satisfy this assumption, see Sec.~\ref{sec:mesh_conversion}). We aim to represent this surface as the $\ell$ level set of a function $F(\mathbf{x}, \theta)$, where $\mathbf{x}$ is a 3D position and $\theta$ is a vector of template parameters. In the structured implicit formulation, $F$ is the sum of the contributions of a fixed number of shape elements with local influence, defined by the parameter vector $\theta$. 




The specific version of this representation we adopt is a collection of Gaussian functions that varying in radius along each 3D axis (anisotropic scaling), with overall strength varying by a scalar factor. Intuitively, one can think this of representation as a set of squished or stretched 3D blobs. We found this set of parameters to be the minimum necessary to achieve good results. More sophisticated shape elements, such as full multivariate Gaussians, or even windowed quadric functions~\cite{ohtake2003multi}, would likely improve results, but we do not experiment with those here.  

Formally, our representation is composed of elements labeled $i\in [N]$, where $N$ is the number of elements. The parameter vector $\theta_i$ for each element $i$ is composed of a center $\mathbf{p}_i \in \mathcal{R}^3$, a per-axis radius $\mathbf{r}_i \in \mathcal{R}^3$, and an always-negative constant $c_i \in \mathcal{R}^-$. Each element defines an anisotropic Gaussian function over all of space:
\begin{equation}
    f_i(\mathbf{x}, \theta_i) = c_i \exp\left({\sum_{d \in \{x,y,z\}} \dfrac{(p_{i,d} - x_d)^2}{-2r_{i,d}^2} }\right)
\end{equation}.

The composition function for the elements is a sum. Therefore, the global function representing the shape is:
\begin{equation}
    F(\mathbf{x}, \theta) = \sum_{i \in [N]} f_i(\mathbf{x}, \theta_i)
\end{equation}
where the parameter vector $\theta$ is simply the concatenation of the $\theta_i$. 

Because all constants $c_i$ are negative, we have that $\forall \mathbf{x} \in \mathcal{R}^3, f_i(\mathbf{x}, \theta) < 0$, and similarly $\forall \mathbf{x} \in \mathcal{R}^3, F(\mathbf{x}, \theta) < 0$. Therefore we pick a negative isolevel $\ell$ and define the surface $S$ to be its crossing:
\begin{equation}
    S = \left\{ \mathbf{x}  \in \mathcal{R}^3 : F(\mathbf{x}, \theta)  = \ell\right\}
\end{equation}

We set $\ell := -0.07$, which was chosen by grid search. The reason that the constants are negative rather than positive is to maintain the convention that function values inside the surface should be less than $\ell$, while values outside the surface should be greater than $\ell$. This leads to a convenient 1/0 outside/inside test for points $x$:

\begin{equation}
    F(\mathbf{x}, \theta) > \ell
\end{equation}

During training, the behavior of gradients is improved by smoothing out the inside/outside function with a sigmoid operation:

\begin{equation}
    \mathrm{Sigmoid}\left(\alpha (F(\mathbf{x}, \theta) - \ell)\right)
    \label{eq:soft_classification}
\end{equation}

where $\alpha$ defines the degree of smoothing out to be applied to the inside/outside query. 

For most experiments presented here, we use $N = 100$. Because each shape element has seven parameters, the total dimensionality of our representation is a fixed $7N = 700$ floating point values. 




==> sections/archive.tex <==

Desirable properties of the shape representation
(maybe put these in a table with check marks for different
representations):
\begin{itemize}
\setlength{\parsep}{0pt}
\setlength{\topsep}{0pt}
\setlength{\itemsep}{0pt}
\item Decomposes a shape into a set of structural/semantic elements
  -- useful for structural/semantic segmentation
\item Consistent across a class of shapes
  -- useful for interpolation, learning, correspondence, matching
\item Human interpretable
  -- useful for editing and visualization
\item Compact
  -- amount of data ~ complexity of shape
\item Learned without supervision
  -- useful for datasets without human labels
\item Can be trained with multiple classes at once
  -- automatically make inter-class associations

\item Handles shapes with detailed structures
  -- can be applied for complex shapes with small parts
\item Handles shapes with arbitrary topology/genus
  -- can be applied for wide range of shape classes
  
\item Can extract surface/volume reconstruction
  -- surface useful for rendering
  -- volume useful for reasoning about inside/outside
  -- Not required, but nice?
\item Differentiable rendering (not now?)
\end{itemize}


==> sections/todos.tex <==

\section{\TODO{}}
TODO RESULTS:
\begin{itemize}


\item Tulsiani Qualitative Comparison Figure. TODO: Clean this figure up.



\item RGB $\rightarrow$ 2D -> Correpondence + 3D Reconstruction Qualitative Results. Daniel's highest priority. (rework and text).


\item QLerp visualization. Needs more text.

\item Results for other classes for us? The teaser.




TODO WRITING:
\item Intro, Related work section. (Tom, Forrester).
\item Method Section. (Kyle, Forrester).
\item Experiments section. (Each person fill in text associated with their figure(s)). 
\item Conclusion (TBD)
\item Abstract (TBD)
\item Comparison to Tulsiani et al? (TBD)
\item Method Figure (TBD)
\item Upload test set results. (Kyle)
\item Enter paper id?


ASSIGNMENTS:
\end{itemize}

==> tab/tab_reconstruction_results_nmr.tex <==
\setlength{\tabcolsep}{2pt}
\begin{table}[t]
\centering
\begin{small}
\begin{tabular}{lcccccccccc}
\toprule
Threshold  & \multicolumn{5}{c}{$\tau$} & \multicolumn{5}{c}{$2\tau$} \\
\cmidrule{2-6} \cmidrule{7-11} \\
Category   & R2N2 & PSG & NMR & P2M & Our       & R2N2 & PSG & NMR & P2M & Our   \\
\midrule
plane      & 41 & 68 & 62 & \textbf{71} & 69    & 63 & 81 & 77 & 81 & \textbf{86} \\
bench      & 34 & 49 & 36 & 58 & \textbf{62}    & 49 & 69 & 50 & 72 & \textbf{82} \\
cabinet    & 50 & 40 & 21 & \textbf{60} & 40    & 65 & 67 & 35 & \textbf{77} & 64  \\
car        & 38 & 51 & 37 & \textbf{68} & 47    & 55 & 78 & 54 & \textbf{84} & 70  \\
chair      & 40 & 42 & 30 & \textbf{54} & 40    & 55 & 64 & 45 & \textbf{70} & 64  \\
monitor    & 34 & 40 & 29 & \textbf{51} & 42    & 48 & 64 & 43 & \textbf{67} & 65  \\
lamp       & 32 & 41 & 28 & \textbf{48} & 32    & 44 & 59 & 39 & \textbf{62} & 52  \\
speaker    & 45 & 32 & 19 & \textbf{49} & 29    & 58 & 57 & 32 & \textbf{66} & 50  \\
firearm    & 28 & 70 & 52 & \textbf{73} & 72    & 47 & 83 & 63 & 83 & \textbf{88}  \\
sofa       & 40 & 37 & 25 & \textbf{52} & 42    & 53 & 63 & 40 & \textbf{70} & \textbf{70}  \\
table      & 44 & 53 & 28 & \textbf{66} & 40    & 59 & 73 & 42 & \textbf{79} & 61  \\
cellphone  & 42 & 56 & 28 & \textbf{70} & 56    & 61 & 80 & 42 & \textbf{83} & 79  \\
watercraft & 37 & 51 & 44 & \textbf{55} & 49    & 52 & 71 & 59 & 70 & \textbf{75}  \\
\midrule
mean       & 39 & 49 & 34 & \textbf{60} & 48    & 55 & 70 & 48 & \textbf{74} & 70  \\
\bottomrule
\end{tabular}
\end{small}
\caption{F-score (\%) on ShapeNet test set. Methods compared are 3D-R2N2~\cite{choy20163d}, Point-Set Generating Networks~\cite{fan2017point}, Pix2Mesh~\cite{choy20163d}, and ours.}
\label{tab:reconstruction_results}
\end{table}
